Keeping Your Distance: Solving Sparse Reward Tasks Using Self-Balancing Shaped Rewards

While using shaped rewards can be beneficial when solving sparse reward tasks, their successful application often requires careful engineering and is problem specific. For instance, in tasks where the agent must achieve some goal state, simple distance-to-goal reward shaping often fails, as it renders learning vulnerable to local optima. We introduce a simple and effective model-free method to learn from shaped distance-to-goal rewards on tasks where success depends on reaching a goal state. Our method introduces an auxiliary distance-based reward based on pairs of rollouts to encourage diverse exploration. This approach effectively prevents learning dynamics from stabilizing around local optima induced by the naive distance-to-goal reward shaping and enables policies to efficiently solve sparse reward tasks. Our augmented objective does not require any additional reward engineering or domain expertise to implement and converges to the original sparse objective as the agent learns to solve the task. We demonstrate that our method successfully solves a variety of hard-exploration tasks (including maze navigation and 3D construction in a Minecraft environment), where naive distance-based reward shaping otherwise fails, and intrinsic curiosity and reward relabeling strategies exhibit poor performance.

==> approach_dep.tex <==
\section{Approach}
\label{sec:approach}

This work aims to introduce a generic class of shaped reward for use in goal-conditioned RL.
As discussed in Section \ref{sec:Motivation}, an obvious candidate is to expose the distance function used to define goal reaching as a shaped reward, since no additional domain knowledge is required and this reward shares its optimal policy with that of the sparse reward.
However, policy optimization when using distance-based rewards is sensitive to local optima.
We identify that a local optimum creates a vicious cycle wherein successive cycles of policy optimization tend to reduce the probability that a better optimum will be discovered.
Using $\rho_{\policy}(\state_T | \goal)$ to denote the distribution of terminal states induced by sampling trajectories from policy $\policy(\action_t | \state_t, \goal)$, we can describe the effect of optimization within a local optimum using the expectation
\begin{equation}
\E_{\state_T,\state'_T\sim\rho_{\policy}(\state_T | \goal)}
\left[
\distance{\sgmap{\state_T}}{\sgmap{\state'_T}}
\right],
\end{equation}
where $\state_T, \state'_T$ are independent samples from $\rho_{\policy}(\state_T | \goal)$.
This expectation captures the variability in the terminal states that the policy reaches when pursuing goal $\goal$.
